Offline Stochastic Shortest Path: Learning, Evaluation and Towards Optimality

Goal-oriented Reinforcement Learning, where the agent needs to reach the goal state while simultaneously minimizing the cost, has received significant attention in real-world applications. Its theoretical formulation, stochastic shortest path (SSP), has been intensively researched in the online setting. Nevertheless, it remains understudied when such an online interaction is prohibited and only historical data is provided. In this paper, we consider the offline stochastic shortest path problem when the state space and the action space are finite. We design the simple value iteration-based algorithms for tackling both offline policy evaluation (OPE) and offline policy learning tasks. Notably, our analysis of these simple algorithms yields strong instance-dependent bounds which can imply worst-case bounds that are near-minimax optimal. We hope our study could help illuminate the fundamental statistical limits of the offline SSP problem and motivate further studies beyond the scope of current consideration.

==> sections/abstract.tex <==
% !TEX root = ../characterize_ope.tex
%\my{The title is too long, feel free to change}
%\red{add a figure for singleton absorbing MDP. add discussion for Constraint MDP.}



%Standard importance-sampling based approaches for this problem suffer from a variance that scales exponentially with time horizon $H$, which motivates a splurge of recent interest in alternatives that break the ``Curse of Horizon'' \citep{liu2018breaking,xie2019towards}. In particular, it was shown that a marginalized importance sampling (MIS) approach can be used to achieve an estimation error of order $O(H^3/ n)$ in mean square error (MSE) under an episodic Markov Decision Process model with finite states and potentially infinite actions.


%but only in the case when the action space is finite. 

%\red{When the action space is unbounded, we prove a stronger information-theoretic lower bound of $\Omega(H^3)$, which certifies that the original MIS estimator is indeed rate-optimal in the large action setting.} 



 

==> sections/application.tex <==
% !TEX root = ../example_paper.tex


For the global switching cost of Algorithm~\ref{algo2}, we have the following conclusion.



We use a lemma from \cite{jin2020reward}. The proof of this lemma is dedicated and we include a proof for self-containedness in Appendix~\ref{appb}.

\begin{lemma}[Lemma C.2 in \cite{jin2020reward}]\label{lem13}
	Suppose $\widehat{\mathbb{P}}$ is the empirical transition matrix formed by sampling according to $\mu$ distribution for $N$ samples, $G$ can be any function from $\mathcal{S}$ to $[0,H]$, $\nu$ can be any function from $\mathcal{S}$ to $\mathcal{A}$, then with probability at least $1-\delta$, we have for any $h\in[H]$:
\begin{align*}	
&\max_{G:\mathcal{S}\rightarrow[0,H]}\max_{\nu:\mathcal{S}\rightarrow\mathcal{A}}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}\\ &\leq O(\frac{H^{2}S\log(HAN/\delta)}{N}).
\end{align*}
\end{lemma}

Recall that $\iota=\log(2HAK/\delta)$. We would like to state that for any policy and reward function, the value function under $\widetilde{P}$ and $\widehat{P}$ are close to each other. The proof of Lemma~\ref{lem14} is deferred to Appendix~\ref{appb}.
\begin{lemma}\label{lem14}
	Conditioned on the fact that $P^{int}$ is $\frac{1}{H}$-multiplicatively accurate to $\widetilde{P}$ (the case in Lemma~\ref{lem6}), with probability $1-\frac{T\delta}{2K}$, for any policy $\pi\in\phi$ and any reward function $r^{\prime}$, $$|V^{\pi}(r^{\prime},\widehat{P})-V^{\pi}(r^{\prime},\widetilde{P})|=O(\sqrt{\frac{H^{5}S^{2}A\iota}{T}}).$$
\end{lemma}







%\newpage

==> sections/proof_overview.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex

%\yub{Maybe ``Proof overview'' as the subtitle?}



Our uniform convergence analysis in Section~\ref{sec:mart_con}, relies on creating an unbiased version of $\widehat{v}_\text{OPEMA}$ (which we call it $\widetilde{v}_\text{OPEMA}$) artificially and use concentration (Lemma~\ref{lem:sufficient_sample}) to guarantee $\widehat{v}_\text{OPEMA}$ is identical to $\widetilde{v}_\text{OPEMA}$ in most situations. By doing so we can reduce our analysis from $\sup_{\pi\in\Pi} \left|\widehat{v}^\pi-v^\pi\right|$ to $\sup_{\pi\in\Pi} \left|\widetilde{v}^\pi-v^\pi\right|$. Specifically, $\widetilde{v}^\pi$ replaces  $\widehat{P}_{t}$, $\widehat{r}_t$ in $\widehat{v}^\pi$ by its fictitious counterparts $\widetilde{P}_{t}$, $\widetilde{r}_t$, defined as:
{\small
	\begin{align*}
	\widetilde{r}_t(s_t,a_t)&=\widehat{r}_t(s_t,a_t)\mathbf{1}(E_t)+{r}_t(s_t,a_t)\mathbf{1}(E_t^c),\\
	\widetilde{P}_{t+1}(\cdot|s_t,a_t)&=\widehat{P}_{t+1}(\cdot|s_t,a_t)\mathbf{1}(E_t)+{P}_{t+1}(\cdot|s_t,a_t)\mathbf{1}(E_t^c).
	\end{align*}
}where $E_t$ denotes the event $\{n_{s_t,a_t}\geq nd^\mu_t(s_t,a_t)/2\}$. This is saying, if observation $n_{s_t,a_t}$ is large enough ($E_t$ is true), we use $\widehat{P}$; otherwise we directly use $P$ instead. This track helps dealing with out-of-sample state-action pairs. The next key is the martingale decomposition (Lemma~\ref{lem:martingale_decompose}). On one hand, by using the structure of {\small $\sup_{\pi\in\Pi}\langle{V^\pi_h,(\widetilde{T}_h-T_h)\widetilde{d}^\pi_{h-1}}\rangle$} we can relax it into a ``Rademacher-type complexity'' which corresponds to $\tilde{O}(\sqrt{H^4S/d_m n})$ term in Theorem~\ref{thm:rad}. On the other hand, this decomposition has a natural martingale structure so martingale concentration inequalities can be appropriately applied, \emph{i.e.} Theorem~\ref{thm:single_finer_bound}. In addition, each term {\small $\langle{V^\pi_h,(\widetilde{T}_h-T_h)\widetilde{d}^\pi_{h-1}}\rangle$} separates the non-stationary policy into two parts with empirical distribution only depends on $\pi_{1:h-1}$ that governs how the data ``roll in'' and the long term value function $V^\pi_h$ only depends on $\pi_{h:H}$ that governs how the reward ``roll out''. 

For local uniform convergence, by Bellman equations we can obtain a similar decomposition on $Q$-function:
{
\begin{align*}
\widehat{Q}^\pi_t-Q^\pi_t&=\sum_{h=t+1}^H \Gamma_{t+1:h-1}^\pi(\widehat{P}_{h}-{P}_{h}) \widehat{V}^\pi_{h},
\end{align*}}
where $\Gamma_{t:h}^\pi=\prod_{i=t}^hP^\pi_i$ is the multi-step state-action transition and $\Gamma_{t+1:t}^\pi:=I$. Since $\pi$ is any policy in ${\Pi}_1$ which may dependent on $\mathcal{D}'$ so we cannot directly apply concentration inequalities on $(\widehat{P}_{h}-{P}_{h}) \widehat{V}^\pi_{h}$. Instead, we overcome this hurdle by doing concentration on $(\widehat{P}_{h}-{P}_{h}) \widehat{V}^{\widehat{\pi}^*}_{h}$ since $\widehat{V}^{\widehat{\pi}^*}_{h}$ and $\widehat{P}_{h}$ are independent, and we connect $\widehat{V}^{\widehat{\pi}^*}_{h}$ back to $\widehat{V}^\pi_{h} $ by using they are $\epsilon_\mathrm{opt}$ close (Theorem~\ref{thm:local_uni_opt}). This idea helps avoiding the technicality of absorbing MDP used in \cite{agarwal2020model} for infinite horizon case because of our non-stationary transition setting. For the uniform convergence lower bound, our analysis relies on reducing the problem to identifying $\epsilon$-optimal policy and proving any algorithm that learns a $\epsilon$-optimal policy requires at least $\Omega(H^3/d_m\epsilon^2)$ episodes in the non-stationary episodic setting. Previously, \cite{jiang2017contextual} proves the $\Omega(HSA/\epsilon^2)$ lower bound with assumption $\sum_{i=1}^Hr_i\leq 1$. Our proof uses a modified version of their hard-to-learn MDP instance to achieve the desired result. To produce extra $H^2$ dependence, we leverage the Assumption~\ref{assume1} that $\sum_{i=1}^Hr_i$ may be of order $O(H)$. We only present the high-level ideas here due the space constraint, detailed proofs are explicated in order in Appendix~\ref{sec:the_uni_crude}, \ref{app_sec:mar}, \ref{sec:E}, \ref{sec:lower}.












%\red{Talk about how CR lower bound might not be asymptotically achievable in some cases.}

==> sections/proofs.tex <==
% !TEX root = ../example_paper.tex
\begin{onecolumn}
\section{Extended related work}\label{appr}
\textbf{Low regret reinforcement learning algorithms}
There has been a long line of works (\cite{brafman2002r}, \cite{kearns2002near}, \cite{jaksch2010near}, \cite{osband2013more}, \cite{agrawal2017posterior}, \cite{jin2018q}) focusing on regret minimization for online reinforcement learning. \citet{azar2017minimax} used model-based algorithm (UCB-Q-values) to achieve the optimal regret bound $\widetilde{O}(\sqrt{HSAT})$ for stationary tabular MDP. \citet{dann2019policy} used algorithm ORLC to match the lower bound of regret and give policy certificates at the same time. \citet{zhang2020almost} used Q-learning type algorithm (UCB-advantage) to achieve the optimal $\widetilde{O}(\sqrt{H^{2}SAT})$ regret for non-stationary tabular MDP. \citet{zanette2019tighter} designed the algorithm EULER to get a problem dependent regret bound.

\par
\textbf{Reward-free exploration}
 \citet{jin2020reward} first studied the problem of reward-free exploration, they used a regret minimization algorithm EULER \cite{zanette2019tighter} to visit each state as much as possible. The sample complexity for their algorithm is $\widetilde{O}(H^{5}S^{2}A/\epsilon^{2})$ episodes. \citet{kaufmann2020adaptive} designed an algorithm RF-UCRL by building upper confidence bound for any reward function and any policy that needs of order $\widetilde{O}((S^{2}AH^{4}/\epsilon^{2})$ episodes to output a near-optimal policy for any reward function with high probability. \citet{menard2020fast} constructed a novel exploration bonus of order $\frac{1}{n}$ and their algorithm achieved sample complexity of $\widetilde{O}((S^{2}AH^{3}/\epsilon^{2})$. \citet{zhang2020nearly} considered a more general setting with stationary transition kernel and uniformly bounded reward. They designed a novel condition to achieve the optimal sample complexity $\widetilde{O}((S^{2}A/\epsilon^{2})$ under their setting. Also, their result can be used to achieve $\widetilde{O}((S^{2}AH^{2}/\epsilon^{2})$ sample complexity under traditional setting where $r_{h}\in [0,1]$, this result matches the lower bound. For linear MDP setting, \citet{wang2020reward} and \citet{zanette2020provably} analyzed reward-free exploration under this setting. There is a similar setting named task-agnostic exploration. \citet{zhang2020task} designed an algorithm: UCB-Zero that finds $\epsilon$-optimal policies for $N$ arbitrary tasks after at most $\widetilde{O} (\log(N)H^{5}SA/\epsilon^{2})$ exploration episodes. 
A concurrent work \cite{towards} analyzed low adaptive reward-free exploration under linear MDP. In our work, we consider low adaptive reward-free exploration under tabular MDP, our switching cost is of the same order as \cite{towards} and our sample complexity is much smaller than theirs if directly plugging in $d=SA$ in their bounds.

\paragraph{Bandit algorithms with limited adaptivity}
There has been a long history of works about multi-armed bandit algorithms with low adaptivity \cite{cesa2013online}, \cite{perchet2016batched}, \cite{gao2019batched}, \cite{esfandiari2019regret}. \citet{cesa2013online} designed an algorithm with $\widetilde{O}(\sqrt{KT})$ regret using $O(\log\log T)$ batches. \citet{perchet2016batched} proved a regret lower bound of  $\Omega(T^{\frac{1}{1-2^{1-M}}})$ for algorithms within $M$ batches under $2$-armed bandit setting, which means $\Omega(\log\log T)$ batches are necessary for a regret bound of $\widetilde{O}(\sqrt{T})$. The result is generalized to $K$-armed bandit by \citet{gao2019batched}. We will show the connection and difference between this setting and the low switching setting. In batched bandit problems, the agent decides a sequence of arms and observes the reward of each arm after all arms in that sequence are pulled. More formally, at the beginning of each batch, the agent decides a list of
arms to be pulled. Afterwards,
a list of (arm,reward) pairs is given to the agent. Then
the agent decides about the next batch. \cite{esfandiari2019regret}. Under the switching cost setting, the algorithm can monitor the data stream and decide to change policy at any time, which means an algorithm with low switching cost can have $\Omega(T)$ batches. In addition, algorithms with limited batches can have large switching cost because in one batch, the algorithm can use different policies. Under batched bandit problem, algorithms with at most $M$ batches can have a $MK$ upper bound for switching cost. However, if we generalize batched bandit to batched RL, algorithms with at most $M$ batches can have $A^{SH}M$ switching cost in the worst case. We conclude that an upper bound of batches and an upper bound of switching cost can not imply each other in the worst case.

\section{Missing algorithm: EstimateTransition (Algorithm~\ref{algo_transition_kernel}) and some explanation}\label{appb1}
\begin{algorithm}
	\caption{Compute Transition Kernel (EstimateTransition)}\label{algo_transition_kernel}
	\begin{algorithmic}[1]
		\STATE \textbf{Require}: Data set $\mathcal{D}$, infrequent tuples $\mathcal{F}$, absorbing state $s^{\dagger}$, the target layer $h$, transition kernel $P$.
		\STATE \textbf{Output}: Estimated transition kernel $P$ from data $\mathcal{D}$.
		\STATE \maroon{$\diamond$ Count the visitation number of each state-action pairs from the target layer $h$:}
		\FOR{$(s,a,s')\in\mathcal{S}\times\mathcal{A}\times\mathcal{S}$}
		\STATE $N_{h}(s,a,s^{\prime})=\text{count of}\ (h,s,a,s^{\prime})$ in $\mathcal{D}$.
		\STATE $N_{h}(s,a)=\text{count of}\ (h,s,a)$ in $\mathcal{D}$.
		\ENDFOR
        \STATE \maroon{$\diamond$ Update the $h$-th layer of the transition kernel:}
		\FOR{$(s,a,s^{\prime})\in \mathcal{S}\times \mathcal{A}\times\mathcal{S}$ s.t. $(h,s,a,s^{\prime})\in \mathcal{F}$}
		\STATE $P_{h}(s^{\prime}|s,a)=0.$
		\ENDFOR
		\FOR{$(s,a,s^{\prime})\in \mathcal{S}\times \mathcal{A}\times\mathcal{S}$ s.t. $(h,s,a,s^{\prime})\notin \mathcal{F}$}
		\STATE $P_{h}(s^{\prime}|s,a)=\frac{N_{h}(s,a,s^{\prime})}{N_{h}(s,a)}.$ 
		\ENDFOR
		\FOR{$(s,a)\in \mathcal{S}\times \mathcal{A}$}
		\STATE $P_{h}(s^{\dagger}|s,a)=1-\sum_{s^{\prime}:(h,s,a,s^{\prime})\notin \mathcal{F}}P_{h}(s^{\prime}|s,a).$
		\ENDFOR
		\FOR{$a\in \mathcal{A}$}
		\STATE $P_{h}(s^{\dagger}|s^{\dagger},a)=1.$
		\ENDFOR
		\STATE \textbf{Return} $P$.
	\end{algorithmic}
\end{algorithm}

Algorithm~\ref{algo_transition_kernel} receives a data set $\mathcal{D}$, a set $\mathcal{F}$ of infrequent tuples, a transition kernel $P$ and a target layer $h$ which we want to update. The goal is to update the $h$-th layer of the input transition kernel $P$ while the remaining layers stay unchanged. The construction of $P_{h}$ is for such tuples in $\mathcal{F}$, the transition kernel $P_{h}(s^{\prime}|s,a)$ is 0. For the states not in $\mathcal{F}$, $P_{h}(s^{\prime}|s,a)$ is the empirical estimate. At last, $P_{h}(s^{\dagger}|s,a)=1-\sum_{s^{\prime}:(h,s,a,s^{\prime})\notin \mathcal{F}}P_{h}(s^{\prime}|s,a)$ holds so that $P_{h}$ is a valid transition kernel. For a better understanding, the construction is similar to the construction of $\widetilde{P}$. We first let $P$ be the empirical estimate based on $\mathcal{D}$, then for $(h,s,a,s^{\prime})\in\mathcal{F}$, we move the probability of $P_{h}(s^{\prime}|s,a)$ to $P_{h}(s^{\dagger}|s,a)$.
\newpage
\section{Transition between original MDP and absorbing MDP}\label{appb2}
For any reward function $r$ defined on the original MDP $P$, we abuse the notation and use it on the absorbing version. We extend the definition as: \\
$$r(s,a) = \begin{cases} r(s,a), &   s\in \mathcal{S},  \\ 0,& s=s^{\dagger}. \end{cases}$$
For any policy $\pi$ defined on the original MDP $P$, we abuse the notation and use it on the absorbing version. We extend the definition as: \\
$$\pi(\cdot|s) = \begin{cases} \pi(\cdot|s), &  s\in \mathcal{S}, \\ \text{arbitrary distribution,} & s=s^{\dagger}. \end{cases}$$
Under this definition of $r$ and $\pi$, the expected reward under the absorbing MDP is fixed because once we enter the absorbing state $s^{\dagger}$, we will not get any more reward, so the policy at $s^{\dagger}$ has no influence on the value function.  For any policy $\pi$ defined under the absorbing MDP, we can directly apply it under the true MDP and analyze its value function because $\pi_{h}(\cdot |s)$ has definition for any $s\in \mathcal{S}$.

\section{Technical lemmas}\label{appt}
\begin{lemma}[Bernstein's inequality]\label{lem3}
	Let $x_{1},\cdots,x_{n}$ be independent bounded random variables such that $\mathbb{E}[x_{i}]=0$ and $|x_{i}|\leq A$ with probability $1$. Let $\sigma^{2}=\frac{1}{n}\sum_{i=1}^{n}Var[x_{i}]$, then with probability $1-\delta$ we have 
	$$|\frac{1}{n}\sum_{i=1}^{n}x_{i}|\leq \sqrt{\frac{2\sigma^{2}log(2/\delta)}{n}}+\frac{2A}{3n}log(2/\delta).$$
\end{lemma}

\begin{lemma}[Empirical Bernstein's inequality]\label{lem4}
	Let $x_{1},\cdots,x_{n}$ be i.i.d random variables such that $|x_{i}|\leq A$ with probability $1$. Let $\overline{x}=\frac{1}{n}\sum_{i=1}^{n}x_{i}$,and $\widehat{V}_{n}=\frac{1}{n}\sum_{i=1}^{n}(x_{i}-\overline{x})^{2}$, then with probability $1-\delta$ we have 
	$$|\frac{1}{n}\sum_{i=1}^{n}x_{i}-\mathbb{E}[x]|\leq \sqrt{\frac{2\widehat{V}_{n}log(2/\delta)}{n}}+\frac{7A}{3n}log(2/\delta).$$
\end{lemma}

\begin{lemma}[Lemma F.4 in \cite{dann2017unifying}]\label{lem7}
Let $F_{i}$ for $i = 1\cdots$ be a filtration and $X_{1},\cdots, X_{n}$ be a sequence of Bernoulli random variables with $\mathbb{P}(X_{i} = 1|F_{i-1}) = P_{i}$ with $P_{i}$ being $F_{i-1}$-measurable and $X_{i}$ being $F_{i}$ measurable. It holds that
$$\mathbb{P}[\exists\, n: \sum_{t=1}^{n}X_{t} < \sum_{t=1}^{n}P_{t}/2-W ]\leq e^{-W}.$$	
\end{lemma}

Recall that $\iota=\log(2HAK/\delta)$.
\begin{lemma}\label{lem8}
	Let $F_{i}$ for $i = 1\cdots$ be a filtration and $X_{1},\cdots, X_{n}$ be a sequence of Bernoulli random variables with $\mathbb{P}(X_{i} = 1|F_{i-1}) = P_{i}$ with $P_{i}$ being $F_{i-1}$-measurable and $X_{i}$ being $F_{i}$ measurable. It holds that
	$$\mathbb{P}[\exists\, n: \sum_{t=1}^{n}X_{t} < \sum_{t=1}^{n}P_{t}/2-\iota ]\leq \frac{\delta}{HAK}. $$	
\end{lemma}

\begin{proof}
	Directly plug in $W=\iota$ in lemma~\ref{lem7}.
\end{proof}


\section{Proof of lemmas in Exploration (About Algorithm~\ref{algo1})}\label{appa}
First, we want to highlight that in this paper, under the absorbing MDP, $\mathcal{S}$ only denotes the original states, the absorbing state $s^{\dagger}\notin \mathcal{S}$.

\begin{lemma}\label{lem1}
	The global switching cost of Algorithm~\ref{algo1} is bounded by $HSA$.
\end{lemma}

\begin{proof}
	There are at most $HSA$ different $\pi_{h,s,a}$'s, Algorithm~\ref{algo1} will just run each policy for several times. 
\end{proof}

Inspired by multiplicative Chernoff bound \cite{chernoff1952measure}, we define 
\begin{definition}[$\theta$-multiplicatively accurate]\label{def30}
	For $\theta<1$, an estimate $\widehat{X}$ of $X$ is $\theta$-multiplicatively accurate iff $$(1-\theta)\widehat{X} \leq X \leq (1+\theta)\widehat{X}.$$
\end{definition}

We extend this definition to transition kernels.
\begin{definition}[$\theta$-multiplicatively accurate]\label{def3}
	A transition model $P^{\prime}$ is $\theta$-multiplicatively accurate to another transition model $P^{\prime\prime}$ iff $$(1-\theta)P^{\prime}_{h}(s^{\prime}|s,a) \leq P^{\prime\prime}_{h}(s^{\prime}|s,a) \leq (1+\theta)P^{\prime}_{h}(s^{\prime}|s,a)$$ for all $(h,s,a,s^{\prime})$.
\end{definition}

\begin{lemma}\label{lem2}
	Define $1_{h,s,a}$ to be the reward function $r^{\prime}$ such that $r^{\prime}_{h^{\prime}}(s^{\prime},a^{\prime})=\mathbb{I}[(h^{\prime},s^{\prime},a^{\prime})=(h,s,a)]$. Similarly, define  $1_{h,s}$ to be the reward function $r^{\prime}$ such that $r^{\prime}_{h^{\prime}}(s^{\prime},a^{\prime})=\mathbb{I}[(h^{\prime},s^{\prime})=(h,s)]$. Then $V^{\pi}(1_{h,s,a},P^{\prime})$ and $V^{\pi}(1_{h,s},P^{\prime})$ denote the visitation probability to $(h,s,a)$ and $(h,s)$, respectively, under $\pi$ and $P^{\prime}$. If $P^{\prime}$ is $\frac{1}{H}$-multiplicatively accurate to $P^{\prime\prime}$, for any policy $\pi$ and any $(h,s,a)$, it holds that
	$$\frac{1}{4}V^{\pi}(1_{h,s,a},P^{\prime}) \leq V^{\pi}(1_{h,s,a},P^{\prime\prime}) \leq 3V^{\pi}(1_{h,s,a},P^{\prime})$$
\end{lemma}

\begin{proof} 
	For any trajectory $\tau=\{s_{1},a_{1},s_{2},a_{2},\cdots,s_{H},a_{H},s_{H+1}\}$, it holds that
	\begin{align*}
	\mathbb{P}_{\pi}[\tau|P^{\prime\prime}]&= \prod_{h=1}^{H}\pi(a_{h}|s_{h})\times \prod_{h=1}^{H}P_{h}^{\prime\prime}(s_{h+1}|s_{h},a_{h}) \\ &\leq (1+\frac{1}{H})^{H}\prod_{h=1}^{H}\pi(a_{h}|s_{h})\times \prod_{h=1}^{H}P_{h}^{\prime}(s_{h+1}|s_{h},a_{h}) \\ &\leq 3\mathbb{P}_{\pi}[\tau|P^{\prime}].
	\end{align*}
	Let $\tau_{h,s,a}$ be the set of trajectories such that $(s_{h},a_{h})=(s,a)$. Then
	$$V^{\pi}(1_{h,s,a},P^{\prime\prime})=\sum_{\tau\in \tau_{h,s,a}}\mathbb{P}_{\pi}[\tau|P^{\prime\prime}]\leq 3\sum_{\tau\in \tau_{h,s,a}}\mathbb{P}_{\pi}[\tau|P^{\prime}]=3V^{\pi}(1_{h,s,a},P^{\prime}).$$
	The left side of the inequality can be proven in a similar way, with $(1-\frac{1}{H})^{H}\geq \frac{1}{4}$ when $H\geq 2$.
\end{proof}

\begin{remark}
For simplicity, in Lemma~\ref{lem2} we only prove under the case that $(1-\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a) \leq P^{\prime\prime}_{h}(s^{\prime}|s,a) \leq (1+\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a)$ for all $(h,s,a,s^{\prime})$. We will generalize Lemma~\ref{lem2} a little in Lemma~\ref{lem26} below.
\end{remark}

\begin{lemma}\label{lem26}
Under the absorbing MDP with absorbing state $s^{\dagger}$, if $(1-\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a) \leq P^{\prime\prime}_{h}(s^{\prime}|s,a) \leq (1+\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a)$ for any $(h,s,a,s^{\prime})\in[H]\times\mathcal{S}\times\mathcal{A}\times\mathcal{S}$ and there is no requirement for the case $s^{\prime}=s^{\dagger}$, we have for any policy $\pi$ and any $(h,s,a)\in [H]\times \mathcal{S}\times \mathcal{A}$, 
$$\frac{1}{4}V^{\pi}(1_{h,s,a},P^{\prime}) \leq V^{\pi}(1_{h,s,a},P^{\prime\prime}) \leq 3V^{\pi}(1_{h,s,a},P^{\prime}).$$
\end{lemma}

\begin{proof}
The proof is almost same to the proof of Lemma~\ref{lem2}. Under the absorbing MDP, for any trajectory $\tau=\{s_{1},a_{1},\cdots,s_{h},a_{h}\}$ (truncated at time step $h$) such that $(s_{h},a_{h})=(s,a)$ and $s\in\mathcal{S}$, we have $s_{h^{\prime}}\neq s^{\dagger}$ for any $h^{\prime}\leq h-1$. Then it holds that for any $\pi$,
$$\frac{1}{4}\mathbb{P}_{\pi}[\tau|P^{\prime}]\leq\mathbb{P}_{\pi}[\tau|P^{\prime\prime}]\leq 3\mathbb{P}_{\pi}[\tau|P^{\prime}].$$ Adding up all the trajectories truncated at step $h$ such that  $(s_{h},a_{h})=(s,a)$, we have for any $\pi$ and any $(h,s,a)\in [H]\times \mathcal{S}\times \mathcal{A}$, 
$$\frac{1}{4}V^{\pi}(1_{h,s,a},P^{\prime}) \leq V^{\pi}(1_{h,s,a},P^{\prime\prime}) \leq 3V^{\pi}(1_{h,s,a},P^{\prime}).$$
\end{proof}

\begin{remark}\label{rem1}
	In this setting, under the absorbing MDP, we will show that with high probability, for any $(h,s,a,s^{\prime})\in [H]\times \mathcal{S}\times \mathcal{A}\times \mathcal{S}$, it holds that
	$ (1-\frac{1}{H})P^{int}_{h}(s^{\prime}|s,a)\leq \widetilde{P}_{h}(s^{\prime}|s,a) \leq (1+\frac{1}{H})P^{int}_{h}(s^{\prime}|s,a). $ However, this may not be true when $s^{\prime}=s^{\dagger}$, the absorbing state. By Lemma~\ref{lem26}, it holds that for any policy $\pi$ and any $(h,s,a)\in [H]\times \mathcal{S}\times \mathcal{A}$, 
	$\frac{1}{4}V^{\pi}(1_{h,s,a},P^{int}) \leq V^{\pi}(1_{h,s,a},\widetilde{P}) \leq 3V^{\pi}(1_{h,s,a},P^{int})$ is true. For the visitation probability to the absorbing state $s^{\dagger}$, this inequality may not be true, but this is not a big deal because we don't need to explore the absorbing state or consider the visitation probability of $s^{\dagger}$. In the later proof, we will abuse definition a little by calling that an absorbing transition model $P^{\prime}$ is $\frac{1}{H}$-multiplicatively accurate to another absorbing transition model $P^{\prime\prime}$ if $(1-\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a) \leq P^{\prime\prime}_{h}(s^{\prime}|s,a) \leq (1+\frac{1}{H})P^{\prime}_{h}(s^{\prime}|s,a)$ for all $(h,s,a,s^{\prime})\in [H]\times \mathcal{S}\times \mathcal{A}\times \mathcal{S}$ and there is no requirement for the case $s^{\prime}=s^{\dagger}$.
\end{remark}

We can bound the difference between $\widetilde{P}$ and $P^{int}$ by empirical Bernstein's inequality (Lemma~\ref{lem4}).
\begin{lemma}\label{lem5}
	 Define the event $\mathcal{W}$ as: $\forall\, (h,s,a,s^{\prime})\notin \mathcal{F}$, $|P^{int}_{h}(s^{\prime}|s,a)-\widetilde{P}_{h}(s^{\prime}|s,a)|\leq \sqrt{\frac{2P^{int}_{h}(s^{\prime}|s,a)\iota}{N_{h}(s,a)}}+\frac{7\iota}{3N_{h}(s,a)}$. Then with probability $1-\frac{S^{2}\delta}{K}$, the event $\mathcal{W}$ holds. In addition, we have that $\forall\, (h,s,a,s^{\prime})\in \mathcal{F}$, $\widetilde{P}_{h}(s^{\prime}|s,a)=P^{int}_{h}(s^{\prime}|s,a)=0.$
\end{lemma}

\begin{proof}
	The first part is because of Lemma~\ref{lem4} and a union bound. The second part is because of Definition~\ref{def2} and the definition of $P^{int}$ in Algorithm~\ref{algo1}.
\end{proof}

\begin{lemma}\label{lem6}
	Conditioned on the event $\mathcal{W}$ in Lemma~\ref{lem5}, for any $(h,s,a,s^{\prime})\notin \mathcal{F}$, it holds that
	$$ (1-\frac{1}{H})P^{int}_{h}(s^{\prime}|s,a)\leq \widetilde{P}_{h}(s^{\prime}|s,a) \leq (1+\frac{1}{H})P^{int}_{h}(s^{\prime}|s,a). $$
\end{lemma}

\begin{proof}
	Because the event $\mathcal{W}$ is true, we have for any $(h,s,a,s^{\prime})\notin \mathcal{F}$, $$|P^{int}_{h}(s^{\prime}|s,a)-\widetilde{P}_{h}(s^{\prime}|s,a)|\leq \sqrt{\frac{2P^{int}_{h}(s^{\prime}|s,a)\iota}{N_{h}(s,a)}}+\frac{7\iota}{3N_{h}(s,a)}.$$
	Also, for any $(h,s,a,s^{\prime})\notin \mathcal{F}$, $N_{h}(s,a,s^{\prime})\geq C_{1}H^{2}\iota$. \\
	Recall that $P^{int}_{h}(s^{\prime}|s,a)=\frac{N_{h}(s,a,s^{\prime})}{N_{h}(s,a)}$, we have
	\begin{align*}
	|P^{int}_{h}(s^{\prime}|s,a)-\widetilde{P}_{h}(s^{\prime}|s,a)|&\leq \sqrt{\frac{2\iota}{N_{h}(s,a,s^{\prime})}}P^{int}_{h}(s^{\prime}|s,a)+\frac{7P^{int}_{h}(s^{\prime}|s,a)\iota}{3N_{h}(s,a,s^{\prime})}\\ &\leq (\sqrt{\frac{2}{C_{1}}}+\frac{7}{3C_{1}H})\cdot\frac{1}{H}P^{int}_{h}(s^{\prime}|s,a) \\&\leq \frac{1}{H}P^{int}_{h}(s^{\prime}|s,a). 
	\end{align*}
	The first inequality is because of the definition of $P^{int}$. The second inequality is because of the definition of $\mathcal{F}$. The last inequality is because of the choice of $C_{1}=6$. \\
	Then the proof is completed by arranging $|P^{int}_{h}(s^{\prime}|s,a)-\widetilde{P}_{h}(s^{\prime}|s,a)|\leq \frac{1}{H}P^{int}_{h}(s^{\prime}|s,a)$.
\end{proof}

\begin{remark}
	From Lemma~\ref{lem6}, we can see that for those tuples $(h,s,a,s^{\prime})$ which have been visited enough times, the estimate of the transition kernel is $\frac{1}{H}$-multiplicatively accurate to the real transition kernel with high probability. In addition, for those states $(h,s,a,s^{\prime})\in \mathcal{F}$, $P^{int}_{h}(s^{\prime}|s,a)=\widetilde{P}_{h}(s^{\prime}|s,a)=0$, so the conclusion in Lemma~\ref{lem6} is true for all $(h,s,a,s^{\prime})\in [H]\times\mathcal{S}\times\mathcal{A}\times\mathcal{S}$, which means that $P^{int}$ is $\frac{1}{H}$-multiplicatively accurate to $\widetilde{P}$ according to our extended definition of $\frac{1}{H}$-multiplicatively accurate in Remark~\ref{rem1}.
\end{remark}
\begin{remark}\label{rem10}

For the sake of clarity, we conclude some useful properties of the absorbing MDP $\widetilde{P}$ and its estimate $P^{int}$. \\
1. Conditioned on the event $\mathcal{W}$, we have that for any policy $\pi$ and any $(h,s,a)\in [H]\times \mathcal{S}\times \mathcal{A}$, 
$$\frac{1}{4}V^{\pi}(1_{h,s,a},P^{int}) \leq V^{\pi}(1_{h,s,a},\widetilde{P}) \leq 3V^{\pi}(1_{h,s,a},P^{int}).$$
2. Because of the definition of $\widetilde{P}$, we have that for any policy $\pi$ and any $(h,s,a)\in [H]\times \mathcal{S}\times \mathcal{A}$, $$V^{\pi}(1_{h,s,a},P)\geq V^{\pi}(1_{h,s,a},\widetilde{P}).$$
\end{remark}

Next, we will define the following bad event and explain the decomposition of its probability.

\begin{definition}[Bad event $\mathcal{B}$ and $\mathcal{B}_{h}$]\label{def4}
	For a trajectory under a MDP and a policy, define $\mathcal{B}$ to be the event where there exists $h$ such that $(h,s_{h},a_{h},s_{h+1})\in \mathcal{F}$.
	Define $\mathcal{B}_{h}$, for $h=1,2,\cdots, H$ to be the event that $(h,s_{h},a_{h},s_{h+1})\in \mathcal{F}$ and $\ \forall\, h^{\prime}\leq h-1$, $(h^{\prime},s_{h^{\prime}},a_{h^{\prime}},s_{h^{\prime}+1})\notin \mathcal{F}$.
\end{definition}

We also need the corresponding bad event under the absorbing MDP, so we extend the definition of bad events to the absorbing MDP.

\begin{remark}
	Similarly, we extend the definition of $\mathcal{B}$ and $\mathcal{B}_{h}$ to the absorbing MDP. The bad event $\mathcal{B}$ means that $s_{H+1}=s^{\dagger}$ and $\mathcal{B}_{h}$ means that $s_{h+1}=s^{\dagger}$ and $\forall\, h^{\prime}\leq h$, $s_{h^{\prime}}\neq s^{\dagger}$. Also, it's clear that $\mathcal{B}$ is the event that the trajectory finally enters $s^{\dagger}$ (the set $\mathcal{F}$ under the true MDP) and $\mathcal{B}_{h}$ is the event that the trajectory first enters $s^{\dagger}$ (the set $\mathcal{F}$ under the true MDP) at time step $h+1$. We have that under a specific MDP, $\mathcal{B}$ is a disjoint union of $\mathcal{B}_{h}$ and $\mathbb{P}(\mathcal{B})=\sum_{h=1}^{H}\mathbb{P}(\mathcal{B}_{h})$.
\end{remark}

We will restate and prove the two parts of Lemma~\ref{lem9} separately.

\begin{lemma}[Restate Lemma~\ref{lem9} first part]
	Conditioned on $\mathcal{W}$ in Lemma~\ref{lem5}, with probability $1-\frac{\delta}{AK}$, $\sup_{\pi\in\phi} P_{\pi}[\mathcal{B}]\leq \frac{168S^{3}A^{2}H^{4}\iota}{T}$. 
\end{lemma}
\begin{proof}
	For the first part, we will prove that $\forall\, h\in [H]$, with probability $1-\frac{\delta}{HAK}$, $\sup_{\pi\in \phi} P_{\pi}[\mathcal{B}_{h}]\leq \frac{168S^{3}A^{2}H^{3}\iota}{T}$. \\
	First, recall that the event $\mathcal{B}_{h}$ means $(h,s_{h},a_{h},s_{h+1})\in \mathcal{F}$ and $\ \forall\, h^{\prime}\leq h-1$, $(h^{\prime},s_{h^{\prime}},a_{h^{\prime}},s_{h^{\prime}+1})\notin \mathcal{F}$ under the original MDP. Also, $\mathcal{B}_{h}$ means that $s_{h+1}=s^{\dagger}$ and $\forall\, h^{\prime}\leq h$, $s_{h^{\prime}}\neq s^{\dagger}$ under the absorbing MDP. We have
	\begin{equation}\label{equ1}
	\begin{split}
	\mathbb{P}_{\pi}[\mathcal{B}_{h}|P]&=\sum_{\tau\in \mathcal{B}_{h}}\mathbb{P}_{\pi}[\tau|P] \\ &=\sum_{\tau_{:h+1}\in \mathcal{B}_{h}}\mathbb{P}_{\pi}[(s_{1},a_{1},\cdots,s_{h},a_{h})|P]P_{h}(s_{h+1}|s_{h},a_{h}) \\ &=\sum_{\tau_{:h+1}\in \mathcal{B}_{h}}\mathbb{P}_{\pi}[(s_{1},a_{1},\cdots,s_{h},a_{h})|\widetilde{P}]P_{h}(s_{h+1}|s_{h},a_{h}) \\ &=\sum_{s\in \mathcal{S},a}V^{\pi}(1_{h,s,a},\widetilde{P})\sum_{s^{\prime}:(h,s,a,s^{\prime})\in \mathcal{F}}P_{h}(s^{\prime}|s,a) \\ &=\sum_{s\in \mathcal{S},a}V^{\pi}(1_{h,s,a},\widetilde{P})\widetilde{P}_{h}(s^{\dagger}|s,a)\\ &=\mathbb{P}_{\pi}[\mathcal{B}_{h}|\widetilde{P}],
	\end{split}
	\end{equation}
	where $\tau_{:h+1}$ in line 2 and line 3 means the trajectory $\tau$ truncated at $s_{h+1}$. Note that we only need to consider the trajectory truncated at $h+1$ because the event $\mathcal{B}_{h}$ only depends on this part of trajectory.
	The third equation is because for $(h,s,a,s^{\prime})\notin \mathcal{F}$, $P=\widetilde{P}$. The fifth equation is because of the definition of $\widetilde{P}$. The last equation is because of the definition of $\mathcal{B}_{h}$ under the absorbing MDP $\widetilde{P}$.\\
	Then because of the first property in Remark~\ref{rem10} we have
	\begin{equation}\label{equ2}
	\begin{split}
	V^{\pi_{h,s,a}}(1_{h,s,a},\widetilde{P})&\geq \frac{1}{4}V^{\pi_{h,s,a}}(1_{h,s,a},P^{int}) \\ &= \frac{1}{4}\sup_{\pi\in \phi}V^{\pi}(1_{h,s,a},P^{int}) \\ &\geq \frac{1}{12}\sup_{\pi\in \phi}V^{\pi}(1_{h,s,a},\widetilde{P}).
	\end{split}
	\end{equation}
	Define $\pi_{h}$ to be a policy that chooses each $\pi_{h,s,a}$ with probability $\frac{1}{SA}$ for any $(s,a)\in \mathcal{S}\times \mathcal{A}$. Then we have 
	\begin{equation}\label{equ3}
	\begin{split}
	V^{\pi_{h}}(1_{h,s,a},\widetilde{P}) &\geq \frac{1}{SA}V^{\pi_{h,s,a}}(1_{h,s,a},\widetilde{P})\\ &\geq \frac{1}{12SA}\sup_{\pi\in \phi}V^{\pi}(1_{h,s,a},\widetilde{P}).
	\end{split}
	\end{equation}
	Note that in our Algorithm~\ref{algo1}, each policy $\pi_{h,s,a}$ will be run for $\frac{T}{HSA}$ episodes. Then for any event $\mathcal{E}$, we have that 
	$$\sum_{s,a}\frac{T}{HSA}\times P_{\pi_{h,s,a}}[\mathcal{E}|\widetilde{P}]=\frac{T}{H}\times P_{\pi_{h}}[\mathcal{E}|\widetilde{P}].$$
	We will assume that running each $\pi_{h,s,a}$ for $\frac{T}{HSA}$ episodes is equivalent to running $\pi_{h}$ for $\frac{T}{H}$ episodes because with Lemma~\ref{lem8}, we can derive the same lower bound for the total number of event $\mathcal{E}$. In the remaining part of the proof, we will analyze assuming we run $\pi_{h}$ for $\frac{T}{H} $ episodes.\\
	With the definition of $\pi_{h}$, we have
	\begin{align*}
	\mathbb{P}_{\pi_{h}}[\mathcal{B}_{h}|P]&=\mathbb{P}_{\pi_{h}}[\mathcal{B}_{h}|\widetilde{P}] \\ &=\sum_{s\in\mathcal{S},a}V^{\pi_{h}}(1_{h,s,a},\widetilde{P})\widetilde{P}_{h}(s^{\dagger}|s,a)\\ &\geq \frac{1}{12SA}\sum_{s\in\mathcal{S},a}\sup_{\pi\in\phi}V^{\pi}(1_{h,s,a},\widetilde{P})\widetilde{P}_{h}(s^{\dagger}|s,a)\\&\geq \frac{1}{12SA}\sup_{\pi\in\phi}\sum_{s\in\mathcal{S},a}V^{\pi}(1_{h,s,a},\widetilde{P})\widetilde{P}_{h}(s^{\dagger}|s,a) \\&=\frac{1}{12SA}\sup_{\pi\in\phi}\mathbb{P}_{\pi}[\mathcal{B}_{h}|\widetilde{P}]\\&=\frac{1}{12SA}\sup_{\pi\in\phi}\mathbb{P}_{\pi}[\mathcal{B}_{h}|P].
	\end{align*}
	The first and the last equation is because of \eqref{equ1}. The first inequality is because of \eqref{equ3}. The second inequality is because the summation of maximum is larger than the maximum of summation.\\
	Suppose $\sup_{\pi\in\phi}\mathbb{P}_{\pi}[\mathcal{B}_{h}|P]\geq\frac{168S^{3}A^{2}H^{3}\iota}{T}$, then we have $$\mathbb{P}_{\pi_{h}}[\mathcal{B}_{h}|P]\geq\frac{1}{12SA}\sup_{\pi\in\phi}\mathbb{P}_{\pi}[\mathcal{B}_{h}|P]\geq \frac{14S^{2}AH^{3}\iota}{T}.$$
	Therefore, by Lemma~\ref{lem8}, with probability $1-\frac{\delta}{HAK}$, $\mathcal{B}_{h}$ occurs for at least $\frac{T}{H}\times \frac{14S^{2}AH^{3}\iota}{2T}-\iota > 6S^{2}AH^{2}\iota$ times during the exploration of the $h$-th layer. However, by the definition of $\mathcal{F}$, at each time step $h$, for each $(s,a,s^{\prime})$, the event $\mathcal{B}_{h}\cap \{(s_{h},a_{h},s_{h+1})=(s,a,s^{\prime})\}$ occurs for at most $6H^{2}\iota$ times, so the event $\mathcal{B}_{h}=\bigcup_{(s,a,s^{\prime})}(\mathcal{B}_{h}\cap \{(s_{h},a_{h},s_{h+1})=(s,a,s^{\prime})\})$ occurs for at most $6S^{2}AH^{2}\iota$ times in total, which leads to contradiction. \\
	As a result, we have $\forall\, h\in [H]$, with probability $1-\frac{\delta}{HAK}$, $\sup_{\pi\in \phi}\mathbb{P}_{\pi}[\mathcal{B}_{h}]\leq \frac{168S^{3}A^{2}H^{3}\iota}{T}$. Combine these $H$ results, because $\mathbb{P}_{\pi}[\mathcal{B}]=\sum_{h=1}^{H}\mathbb{P}_{\pi}[\mathcal{B}_{h}]$, we have with probability $1-\frac{\delta}{AK}$, 
	$$\sup_{\pi\in \phi}\mathbb{P}_{\pi}[\mathcal{B}]\leq \frac{168S^{3}A^{2}H^{4}\iota}{T}.$$
\end{proof}

The second part of Lemma~\ref{lem9} is an improved version of the first part under the special case where $\phi=\phi^{1}$.
\begin{lemma}[Restate Lemma~\ref{lem9} second part]
	Conditioned on $\mathcal{W}$ in Lemma~\ref{lem5}, if $\phi=\phi^{1}=\{\text{the set of all deterministic policies}\}$, with probability $1-\frac{2S\delta}{K}$, $\sup_{\pi\in\phi^{1}} P_{\pi}[\mathcal{B}]\leq \frac{672S^{3}AH^{4}\iota}{T}$.
\end{lemma}
\begin{proof}
	For the second part, we will prove that $\forall\, h\in [H]$, with probability $1-\frac{2S\delta}{HK}$, $\sup_{\pi\in \phi^{1}} P_{\pi}[\mathcal{B}_{h}]\leq \frac{672S^{3}AH^{3}\iota}{T}$. \\
	First, same to~\eqref{equ1} and~\eqref{equ2} we have
$$	\mathbb{P}_{\pi}[\mathcal{B}_{h}|P]=\mathbb{P}_{\pi}[\mathcal{B}_{h}|\widetilde{P}]. $$
$$ V^{\pi_{h,s,a}}(1_{h,s,a},\widetilde{P})\geq \frac{1}{12}\sup_{\pi\in \phi^{1}}V^{\pi}(1_{h,s,a},\widetilde{P}).$$
Same to the first part, we define $\pi_{h}$ to be a policy that chooses each $\pi_{h,s,a}$ with probability $\frac{1}{SA}$ for any $(s,a)\in \mathcal{S}\times \mathcal{A}$. Then same to~\eqref{equ3}, we have 
$$V^{\pi_{h}}(1_{h,s,a},\widetilde{P})\geq \frac{1}{12SA}\sup_{\pi\in \phi^{1}}V^{\pi}(1_{h,s,a},\widetilde{P})=\frac{1}{12SA}\sup_{\pi\in \phi^{1}}V^{\pi}(1_{h,s},\widetilde{P}).$$
The last equation is because $\phi^{1}$ consists of all the deterministic policies, for the optimal policy $\pi$ to visit $(h,s)$, we can just let $\pi_{h}(s)=a$ to construct a policy that can visit $(h,s,a)$ with the same probability. Because of the same reason in the first part, we can assume that running each $\pi_{h,s,a}$ for $\frac{T}{HSA}$ episodes is equivalent to running $\pi_{h} $ for $\frac{T}{H}$ episodes.\\
According to property 2 in Remark~\ref{rem10}, we have $ V^{\pi_{h}}(1_{h,s,a},P)\geq V^{\pi_{h}}(1_{h,s,a},\widetilde{P})$. Also, there are $\frac{T}{H}$ episodes used to explore the $h$-th layer of the MDP, by Lemma~\ref{lem8} and a union bound, we have with probability $1-\frac{S\delta}{HK}$, $$N_{h}(s,a)\geq \frac{T}{H}\times \frac{V^{\pi_{h}}(1_{h,s,a},P)}{2}-\iota\geq \frac{T}{H}\times \frac{V^{\pi_{h}}(1_{h,s,a},\widetilde{P})}{2}-\iota\geq \frac{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}{24HSA}-\iota,$$ for any $(s,a)\in \mathcal{S}\times\mathcal{A}$. For fixed $(s,a)\in\mathcal{S}\times\mathcal{A}$, if $\frac{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}{24HSA}\leq 2\iota$, we have that 
$$\sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})\leq \frac{48HSA\iota}{T}.$$
Otherwise, $N_{h}(s,a)\geq \frac{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}{48HSA}$. \\
By Lemma~\ref{lem8} and a union bound, we have with probability $1-\frac{S\delta}{HK}$, for any $(s,a)\in \mathcal{S}\times\mathcal{A}$, $6SH^{2}\iota\geq \frac{N_{h}(s,a)P[\mathcal{F}|(h,s,a)]}{2}-\iota$, where $P[\mathcal{F}|(h,s,a)]$ is the conditional probability of entering $\mathcal{F}$ at time step $h$, given the state-action pair at time step $h$ is $(s,a)$. This is because similar to the proof of the first part, the event of entering $\mathcal{F}$ from $(h,s,a)$ happens for at most $6SH^{2}\iota$ times.\\
We have with probability $1-\frac{2S\delta}{HK}$, $\sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})\leq \frac{48HSA\iota}{T}$ or $P[\mathcal{F}|(h,s,a)]\leq\frac{672H^{3}S^{2}A\iota}{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}$ holds for any $(s,a)\in \mathcal{S}\times\mathcal{A}$. \\
Therefore, it holds that
\begin{align*}
\sup_{\pi\in\phi^{1}}\mathbb{P}_{\pi}[\mathcal{B}_{h}|P]&=\sup_{\pi\in\phi^{1}}\mathbb{P}_{\pi}[\mathcal{B}_{h}|\widetilde{P}] \\ &=\sup_{\pi\in\phi^{1}}\sum_{s\in\mathcal{S}}V^{\pi}(1_{h,s},\widetilde{P})\max_{a\in\mathcal{A}}\widetilde{P}_{h}(s^{\dagger}|s,a)\\ & =\sup_{\pi\in\phi^{1}}\sum_{s\in\mathcal{S}}V^{\pi}(1_{h,s},\widetilde{P})\max_{a\in\mathcal{A}}P[\mathcal{F}|(h,s,a)]\\&\leq \sup_{\pi\in\phi^{1}}\sum_{s\in\mathcal{S}}\max\{\frac{48HSA\iota}{T},\frac{672H^{3}S^{2}A\iota}{T}\} \\&=\frac{672H^{3}S^{3}A\iota}{T}.
\end{align*}
The inequality is because if $\frac{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}{24HSA}\leq 2\iota$, 
$$V^{\pi}(1_{h,s},\widetilde{P})\max_{a\in\mathcal{A}}P[\mathcal{F}|(h,s,a)]\leq V^{\pi}(1_{h,s},\widetilde{P})\leq \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})\leq \frac{48HSA\iota}{T}.$$
Otherwise we have that 
$$V^{\pi}(1_{h,s},\widetilde{P})\max_{a\in\mathcal{A}}P[\mathcal{F}|(h,s,a)]\leq V^{\pi}(1_{h,s},\widetilde{P})\frac{672H^{3}S^{2}A\iota}{T\cdot \sup_{\pi\in\phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})}\leq \frac{672H^{3}S^{2}A\iota}{T}.$$
As a result, we have $\forall\, h\in [H]$, with probability $1-\frac{2S\delta}{HK}$, $\sup_{\pi\in \phi^{1}}\mathbb{P}_{\pi}[\mathcal{B}_{h}]\leq \frac{672S^{3}AH^{3}\iota}{T}$. Combine these $H$ results, because $\mathbb{P}_{\pi}[\mathcal{B}]=\sum_{h=1}^{H}\mathbb{P}_{\pi}[\mathcal{B}_{h}]$, we have with probability $1-\frac{2S\delta}{K}$, 
$$\sup_{\pi\in \phi^{1}}\mathbb{P}_{\pi}[\mathcal{B}]\leq \frac{672S^{3}AH^{4}\iota}{T}.$$
\end{proof}

\begin{remark}
We can see that with the same algorithm, the analysis is different for the general case and the special case that $\phi$ contains all the deterministic policies. The main technical reason is when $\phi=\phi^{1}$, $\sup_{\pi\in \phi^{1}}V^{\pi}(1_{h,s,a},\widetilde{P})=\sup_{\pi\in \phi^{1}}V^{\pi}(1_{h,s},\widetilde{P})$ while this does not hold for general policy set $\phi$. We will show that the regret because of constructing $\widetilde{P}$ is a lower order term. We prove a better bound for the case $\phi=\phi^{1}$ mainly for a better sample complexity in reward-free setting. 
\end{remark}

\begin{lemma}[Restate Lemma~\ref{lem10}]
	Conditioned on the event in Lemma~\ref{lem9}, we have $0\leq V^{\pi}(r^{\prime},P)-V^{\pi}(r^{\prime},\widetilde{P})\leq \frac{168S^{3}A^{2}H^{5}\iota}{T}$ holds for any policy $\pi\in\phi$ and reward function $r^{\prime}$. In addition, if $\phi=\phi^{1}=\{\text{the set of all deterministic policies}\}$, we have that $0\leq V^{\pi}(r^{\prime},P)-V^{\pi}(r^{\prime},\widetilde{P})\leq \frac{672S^{3}AH^{5}\iota}{T}$ holds for any policy $\pi\in\phi^{1}$ and reward function $r^{\prime}$.
\end{lemma}

\begin{proof}
	We will only prove the first part, the second part is almost the same. Because $\widetilde{P}$ is the absorbing version of $P$, the left hand side is obvious. For the right hand side, we have that if $\pi\in\phi$,
\begin{align*}
V^{\pi}(r^{\prime},P)&=\sum_{\tau\in \mathcal{B}^{c}}r^{\prime}(\tau)P_{\pi}(\tau)+\sum_{\tau\in \mathcal{B}}r^{\prime}(\tau)P_{\pi}(\tau) \\
&=\sum_{\tau\in \mathcal{B}^{c}}r^{\prime}(\tau)\widetilde{P}_{\pi}(\tau)+\sum_{\tau\in \mathcal{B}}r^{\prime}(\tau)P_{\pi}(\tau) \\ &\leq V^{\pi}(r^{\prime},\widetilde{P})+\sum_{\tau\in \mathcal{B}}r^{\prime}(\tau)P_{\pi}(\tau)\\ &\leq V^{\pi}(r^{\prime},\widetilde{P})+\sum_{\tau\in \mathcal{B}}HP_{\pi}(\tau) \\ &\leq V^{\pi}(r^{\prime},\widetilde{P})+HP_{\pi}(\mathcal{B})\\ &\leq V^{\pi}(r^{\prime},\widetilde{P})+\frac{168S^{3}A^{2}H^{5}\iota}{T}.
\end{align*}
The second equation is because conditioned on $\mathcal{B}^{c}$, $\widetilde{P}=P$. The first inequality is because conditioned on $\mathcal{B}^{c}$, the reward under $P$ and $\widetilde{P}$ are the same. The last inequality is because of Lemma~\ref{lem9}.
\end{proof}

\begin{remark}
	From Lemma~\ref{lem10}, we can see that the existence of the whole set $\mathcal{F}$ has little influence on the value function in the sense that the value functions (of any policy and any reward function) under the real MDP $P$ and the absorbing version $\widetilde{P}$ are close to each other. In conclusion, we get an absorbing MDP $\widetilde{P}$ that is close to the true MDP, and we have a $\frac{1}{H}$-multiplicatively accurate estimate $P^{int}$ of this $\widetilde{P}$.
\end{remark}

\begin{remark}
The idea of proof is that for trajectory $\{s_{1},a_{1},\cdots,s_{H+1}\}$ under the true MDP without reaching the infrequent set $\mathcal{F}$, this same trajectory will not reach the absorbing state $s^{\dagger}$ under the absorbing MDP. The key point is that the expected reward and probability of this trajectory will be the same under the true MDP and the absorbing MDP. The difference of the remaining trajectories can be bounded by $H\sup_{\pi\in \phi}\mathbb{P}_{\pi}[\mathcal{B}]$.
\end{remark}

\section{Proof of lemmas in Evaluation (About Algorithm~\ref{algo2})}\label{appb}
\begin{lemma}\label{lem11}
	The global switching cost of Algorithm~\ref{algo2} is bounded by HSA.
\end{lemma}

\begin{proof}
	There are at most $HSA$ different $\pi_{h,s,a}$'s, Algorithm~\ref{algo2} will just run each policy for several times. 
\end{proof}

\begin{lemma}[Simulation lemma]\label{lem12}
	For any two MDPs $M^{\prime}$ and $M^{\prime\prime}$ with rewards $r^{\prime}$ and $r^{\prime\prime}$ and transition probabilities $\mathcal{P}^{\prime}$ and $\mathcal{P}^{\prime\prime}$, the difference in values $V^{\prime}$, $V^{\prime\prime}$ with respect to the same policy $\pi$ can be written as 
	$$V_{h}^{\prime}(s)-V_{h}^{\prime\prime}(s)=\mathbb{E}_{M^{\prime\prime},\pi}[\sum_{i=h}^{H}[r_{i}^{\prime}(s_{i},a_{i})-r_{i}^{\prime\prime}(s_{i},a_{i})+(\mathbb{P}_{i}^{\prime}-\mathbb{P}_{i}^{\prime\prime})V_{i+1}^{\prime}(s_{i},a_{i})]|s_{h}=s].$$
\end{lemma}

Now we can prove that value functions under $\widetilde{P}$ and $\widehat{P}$ are close to each other.
\begin{lemma}[Restate Lemma~\ref{lem14}]
	Conditioned on the fact that $P^{int}$ is $\frac{1}{H}$-multiplicatively accurate to $\widetilde{P}$ (the case in Lemma~\ref{lem6}), with probability $1-\frac{T\delta}{2K}$, for any policy $\pi\in\phi$ and reward function $r^{\prime}$, $$|V^{\pi}(r^{\prime},\widehat{P})-V^{\pi}(r^{\prime},\widetilde{P})|=O(\sqrt{\frac{H^{5}S^{2}A\iota}{T}}).$$
\end{lemma}

\begin{proof}
	In this part of proof, I will use the notation $V^{\pi}(r^{\prime},\widehat{P})$ to denote the value function under the MDP with reward function $r^{\prime}$ and transition probability $\widehat{P}$. According to simulation lemma (Lemma~\ref{lem12}), we have that $\forall\,\pi\in\phi$,
	\begin{equation}\label{equ4}
	|V^{\pi}(r^{\prime},\widehat{P})-V^{\pi}(r^{\prime},\widetilde{P})|\leq \mathbb{E}_{\widetilde{P}}^{\pi}\sum_{h=1}^{H}|(\widehat{P}_{h}-\widetilde{P}_{h})\cdot\widehat{V}_{h+1}|, \\
	\end{equation}
	where $\widehat{V}$ is the value function under $\widehat{P}$ and $r^{\prime}$. The proof holds simultaneously for all reward function $r^{\prime}$, so I will omit $r^{\prime}$ for simplicity. \\
	Then we have
	\begin{align*}
	&\mathbb{E}_{\widetilde{P}}^{\pi}|(\widehat{P}_{h}-\widetilde{P}_{h})\cdot\widehat{V}_{h+1}|= \sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|V^{\pi}(1_{h,s,a},\widetilde{P}) \\ &\leq \sqrt{\sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}V^{\pi}(1_{h,s,a},\widetilde{P})} \\ &= \sqrt{\sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}V^{\pi}(1_{h,s,a},\widetilde{P})\mathbb{I}\{a=\pi_{h}(s)\}}.
	\end{align*}
	The first equation is because if the trajectory arrives at the absorbing state $s^{\dagger}$ at time step $h$, then the $\widehat{V}_{h+1}(s^{\dagger})$ will be 0. The first inequality is because of Cauchy-Schwarz inequality. The last equation is because for any $\pi\in\phi$, $\pi$ is deterministic.\\
	Define $\pi_{random}$ to be a policy that chooses each $\pi_{h,s,a}$ with probability $\frac{1}{HSA}$ for any $(h,s,a)\in [H]\times\mathcal{S}\times \mathcal{A}$. Define $\mu_{h}(s,a)$ to be $\mu_{h}(s,a)=V^{\pi_{random}}(1_{h,s,a},\widetilde{P})$. Then similar to~\eqref{equ2} and~\eqref{equ3}, we have 
\begin{equation}\label{equ6}
\sup_{\pi\in\phi}\frac{V^{\pi}(1_{h,s,a},\widetilde{P})}{\mu_{h}(s,a)}\leq12HSA.
\end{equation}
	Plugging in this result into the previous inequality, we have
	\begin{align*}
	\mathbb{E}_{\widetilde{P}}^{\pi}|(\widehat{P}_{h}-\widetilde{P}_{h})\cdot\widehat{V}_{h+1}|&\leq\sqrt{\sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}V^{\pi}(1_{h,s,a},\widetilde{P})\mathbb{I}\{a=\pi_{h}(s)\}}\\ &\leq
	\sqrt{\sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}\cdot 12HSA\mu_{h}(s,a)\cdot \mathbb{I}\{a=\pi_{h}(s)\}} \\&\leq \sqrt{12HSA\cdot \sup_{\nu:s\rightarrow a}\sum_{a,s\in \mathcal{S}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}\mu_{h}(s,a)\cdot \mathbb{I}\{a=\nu(s)\}} \\&=\sqrt{12HSA\cdot \sup_{\nu:s\rightarrow a}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})\widehat{V}_{h+1}^{\pi}(s,a)|^{2}\cdot \mathbb{I}\{a=\nu(s)\}}\\&\leq \sqrt{12HSA\cdot \sup_{G:\mathcal{S}\rightarrow[0,H]}\sup_{\nu:s\rightarrow a}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\widetilde{\mathbb{P}}_{h})G  (s,a)|^{2}\cdot \mathbb{I}\{a=\nu(s)\}}.
	\end{align*}
	Because the real data comes from distribution $\mu_{h}^{\prime}(s,a)=V^{\pi_{random}}(1_{h,s,a},P)$ and we have $\mu_{h}^{\prime}(s,a)\geq\mu_{h}(s,a)$ for any $(h,s,a)\in [H]\times\mathcal{S}\times\mathcal{A}$ (because of property 2 in Remark~\ref{rem10}), by Lemma~\ref{lem13} we have with probability $1-\frac{T\delta}{2K}$, for any policy $\pi\in\phi$ and reward function $r^{\prime}$,
	$$\mathbb{E}_{\widetilde{P}}^{\pi}|(\widehat{P}_{h}-\widetilde{P}_{h})\cdot\widehat{V}_{h+1}|=O(\sqrt{\frac{H^{3}S^{2}A\iota}{T}}).$$
	By~\eqref{equ4}, we have that the following conclusion holds for any policy $\pi\in\phi$ and reward function $r^{\prime}$.
	$$|V^{\pi}(r^{\prime},\widehat{P})-V^{\pi}(r^{\prime},\widetilde{P})|=O(\sqrt{\frac{H^{5}S^{2}A\iota}{T}}).$$
\end{proof}

\begin{lemma}[Lemma C.2 in \cite{jin2020reward}]\label{lem13}
	Suppose $\widehat{\mathbb{P}}$ is the empirical transition matrix formed by sampling according to $\mu$ distribution for $N$ samples, $G$ can be any function from $\mathcal{S}$ to $[0,H]$, $\nu$ can be any function from $\mathcal{S}$ to $\mathcal{A}$, then with probability at least $1-\delta$, we have for any $h\in[H]$:
\begin{align*}	
&\max_{G:\mathcal{S}\rightarrow[0,H]}\max_{\nu:\mathcal{S}\rightarrow\mathcal{A}}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}\leq O(\frac{H^{2}S\log(HAN/\delta)}{N}).
\end{align*}
\end{lemma}

\begin{proof}
For completeness and clarity, we rewrite the proof for this lemma in a clearer way. \\
Define random variables
$$X=(\widehat{\mathbb{P}}_{h}G(s,a)-G(s^{\prime}))^{2}-(\mathbb{P}_{h}G(s,a)-G(s^{\prime}))^{2},$$
$$\overline{X}=(f(s,a)-G^{\prime}(s^{\prime}))^{2}-(g(s,a)-G^{\prime}(s^{\prime}))^{2},$$ 
$$Y=X\mathbb{I}\{a=\nu(s)\},\,\overline{Y}=\overline{X}\mathbb{I}\{a=\nu^{\prime}(s)\},$$ 
where $(s,a,s^{\prime})\sim\mu_{h}\times\mathbb{P}_{h}(\cdot|s,a)$.
 Here, $\nu^{\prime}$ can be any function from $\mathbb{S}$ to $\mathbb{A}$ (in equation \eqref{equ10}) and will be the same as $\nu$ in equation~\eqref{equ9},~\eqref{equ8},~\eqref{equ11}. Also, $f$, $g$ and $G^{\prime}$ can be any function (in equation~\eqref{equ10}) from the $\epsilon$-cover defined later and will be the closest function from the $\epsilon$-cover to $\widehat{\mathbb{P}}G(s,a)\mathbb{I}\{a=\nu(s)\}$, $\mathbb{P}G(s,a)\mathbb{I}\{a=\nu(s)\}$ and $G$ in equation~\eqref{equ9},~\eqref{equ8},~\eqref{equ11}.
Also, we define
$$X_{i}=(\widehat{\mathbb{P}}_{h}G(s_{i},a_{i})-G(s_{i}^{\prime}))^{2}-(\mathbb{P}_{h}G(s_{i},a_{i})-G(s_{i}^{\prime}))^{2},$$
$$\overline{X}_{i}=(f(s_{i},a_{i})-G^{\prime}(s_{i}^{\prime}))^{2}-(g(s_{i},a_{i})-G^{\prime}(s_{i}^{\prime}))^{2},$$ 
$$Y_{i}=X_{i}\mathbb{I}\{a_{i}=\nu(s_{i})\},\,\overline{Y}_{i}=\overline{X}_{i}\mathbb{I}\{a_{i}=\nu^{\prime}(s_{i})\},$$ where $(s_{i},a_{i},s_{i}^{\prime})$ is the i-th sample in time step $h$ we collect. Notice that for every tuple $(v^{\prime},f,g,G^{\prime})$ and $\overline{Y}$, $\overline{Y}_{i}$ related to this tuple, we have that $\overline{Y}_{i}$'s are i.i.d samples from the distribution of $\overline{Y}$.\\
Same to the proof in \cite{jin2020reward}, we have these three properties of $Y$ and $Y_{i}$. \\
$$(1)\,\mathbb{E}Y=\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}.$$
$$(2)\,\sum_{i=1}^{N}Y_{i}\leq 0.$$
$$(3)\,Var\{Y\}\leq 4H^{2}\mathbb{E}(Y).$$
Since we are taking maximum over $\nu$ and $G(s)$, and $\widehat{\mathbb{P}}$ is random, we need to cover all the possible $\nu$ and all the possible values of $\widehat{\mathbb{P}}G(s,a)\mathbb{I}\{a=\nu(s)\}$, $\mathbb{P}G(s,a)\mathbb{I}\{a=\nu(s)\}$ and $G$ to $\epsilon$ accuracy to use Bernstein's inequality for the functions in the cover. For $\nu$, there are $A^{S}$ deterministic policies in total. Given a fixed $\nu$, $\widehat{\mathbb{P}}G(s,a)\mathbb{I}\{a=\nu(s)\}$, $\mathbb{P}G(s,a)\mathbb{I}\{a=\nu(s)\}$ and $G$ can be covered by $(H/\epsilon)^{3S}$ values because the first two functions can be covered by $(H/\epsilon)^{2S}$ values (for $a\neq \nu(s)$ the first two will be $0$) and $G$ itself can be covered by $(H/\epsilon)^{S}$ values. \\
By Bernstein's inequality (Lemma~\ref{lem3}) and a union bound, we have with probability $1-\delta$, for any $(\nu^{\prime},f,g,G^{\prime})$ in the $\epsilon$-cover, it holds that
\begin{equation}\label{equ10}
    \mathbb{E}(\overline{Y})-\frac{1}{N}\sum_{i=1}^{N}\overline{Y}_{i}\leq \sqrt{\frac{2Var\{\overline{Y}\}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{N}}+\frac{H^{2}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{3N}.
\end{equation}
Under this high probability case, for any $G$, $\nu$ and $\widehat{\mathbb{P}}$, choose $\nu^{\prime}=\nu$ and $(f,g,G^{\prime})$ to be the closest function from the $\epsilon$-cover to  $\widehat{\mathbb{P}}G(s,a)\mathbb{I}\{a=\nu(s)\}$, $\mathbb{P}G(s,a)\mathbb{I}\{a=\nu(s)\}$ and $G$. Let $\overline{Y}$ be defined according to this $(\nu,f,g,G^{\prime})$. Then we have
\begin{equation}\label{equ9}
    |Y-\overline{Y}|\leq 4H\epsilon,
\end{equation}
for any possible $(s,a,s^{\prime})$ (hence this inequality is also true when adding expectation to both terms) and
\begin{equation}\label{equ8}
\begin{split}
    |Var\{Y\}-Var\{\overline{Y}\}|&\leq |\mathbb{E}(\overline{Y}^{2})-\mathbb{E}(Y^{2})|+|(\mathbb{E}\overline{Y})^{2}-(\mathbb{E}Y)^{2}| \\&\leq 2H^{2}\cdot 4H\epsilon+2H^{2}\cdot 4H\epsilon\\&=16H^{3}\epsilon.
\end{split}
\end{equation}
As a result, we have
\begin{equation}\label{equ11}
\begin{split}
&\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}=\mathbb{E}Y\\&\leq \mathbb{E}Y-\frac{1}{N}\sum_{i=1}^{N}Y_{i} \\&\leq \mathbb{E}\overline{Y}-\frac{1}{N}\sum_{i=1}^{N}\overline{Y}_{i}+8H\epsilon \\&\leq \sqrt{\frac{2Var\{\overline{Y}\}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{N}}+\frac{H^{2}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{3N}+8H\epsilon \\&\leq \sqrt{\frac{2Var\{Y\}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{N}}+\frac{H^{2}\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{3N}\\&+8H\epsilon+\sqrt{\frac{2\cdot 16H^{3}\epsilon\log((\frac{H}{\epsilon})^{3S}\cdot A^{S}\cdot \frac{H}{\delta})}{N}}.
\end{split}
\end{equation}
The first inequality is because of property 2. The second inequality is because of \eqref{equ9}. The third inequality is because of \eqref{equ10}. The last inequality is because of \eqref{equ8} and $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$.\\
We can simply choose $\epsilon=\frac{HS}{32N}$ and plug in property (3) of $Y$, then by solving the following quadratic inequality we can finish the proof.
\begin{equation}
\begin{split}
&\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}\\& \leq\sqrt{\frac{8H^{2}\mathbb{E}_{\mu_{h}}|(\widehat{\mathbb{P}}_{h}-\mathbb{P}_{h})G(s,a)|^{2}\mathbb{I}\{a=\nu(s)\}\cdot 3S\log(\frac{32HAN}{\delta})}{N}}+\frac{2H^{2}S\log(\frac{32HAN}{\delta})}{N}.
\end{split}
\end{equation}
\end{proof}

\section{Proof of lemmas in Adaptive Policy Elimination (Theorem~\ref{the1})}\label{appc}
We first give a proof for the upper bound on the number of stages.
\begin{lemma}\label{lem50}
If $T^{(k)}=K^{1-\frac{1}{2^{k}}}$ for $k=1,2\cdots$, we have 
$$K_{0}=\min\{j:2\sum_{k=1}^{j}T^{(k)}\geq K\}=O(\log\log K).$$
\end{lemma}

\begin{proof}
    Take $j=\log_{2}\log_{2}K$, we have $2T^{(j)}=2\frac{K}{K^{(\log_{2}K)^{-1}}}=2\frac{K}{2}=K$, which means that $$K_{0}\leq \log_{2}\log_{2}K=O(\log\log K).$$
\end{proof}

\begin{lemma}\label{lem15}
	The total global switching cost of Algorithm~\ref{algo3} is bounded by $O(HSA\log\log(T))$.
\end{lemma}

\begin{proof}
	For each stage, the global switching cost is bounded by $2HSA$ because of Lemma~\ref{lem1} and Lemma~\ref{lem11}. There are $O(\log\log T)$ stages. So the total global switching cost is at most $O(HSA\log\log T)$.
\end{proof}
Recall that $\iota=\log(2HAK/\delta)$.
\begin{lemma}[Restate Lemma~\ref{lem16}]
	There exists a constant $C$, such that conditioned on the cases in Lemma~\ref{lem10} and Lemma~\ref{lem14} for all $k$, for any $k$ and $\pi\in\phi^{k}$, we have 
	$$|V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,P)|\leq C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).$$
	In addition, the probability of this case is at least $1-\delta$.
\end{lemma}	

\begin{proof}
\begin{equation}
\begin{split}
|V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,P)|\leq |V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,\widetilde{P}^{k})| +|V^{\pi}(r,\widetilde{P}^{k})-V^{\pi}(r,P)|.
\end{split}
\end{equation}
As a result, when the cases in Lemma~\ref{lem10} and Lemma~\ref{lem14} hold for all $k$, we have this inequality holds. \\
The failure probability is bounded by $(\frac{S^{2}\delta}{K}+\frac{\delta}{AK})\times O(\log\log K)+\sum_{k=1}^{K_{0}}\frac{T^{(k)}\delta}{2K}\leq \delta$ if $K\geq \widetilde{\Omega}(S^{2})$.
\end{proof}

\begin{lemma}\label{lem17}
	Conditioned on the case in Lemma~\ref{lem16}, the optimal policy $\pi^{*}$ will never be eliminated.
\end{lemma}	

\begin{proof}
	For optimal policy $\pi^{*}$, we have
	\begin{align*}
	&\sup_{\widehat{\pi}\in\phi^{k}}V^{\widehat{\pi}}(r,\widehat{P}^{k})-V^{\pi^{*}}(r,\widehat{P}^{k})=V^{\widehat{\pi}^{k}}(r,\widehat{P}^{k})-V^{\pi^{*}}(r,\widehat{P}^{k})\\ &\leq |V^{\widehat{\pi}^{k}}(r,\widehat{P}^{k})-V^{\widehat{\pi}^{k}}(r,P)|+V^{\widehat{\pi}^{k}}(r,P)-V^{\pi^{*}}(r,P)+|V^{\pi^{*}}(r,P)-V^{\pi^{*}}(r,\widehat{P}^{k})|\\&\leq 2C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).
	\end{align*}
	The last inequality is because of Lemma~\ref{lem16} and $\pi^{*}$ is the optimal policy.
\end{proof}

\begin{lemma}\label{lem18}
	Conditioned on Lemma~\ref{lem16}, for the policies that have not been eliminated at stage $k$, i.e. $\pi\in\phi^{k+1}$, we have that
	$$V^{\pi^{*}}(r,P)-V^{\pi}(r,P)\leq 4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).$$
\end{lemma}

\begin{proof}
	For $\pi\in\phi^{k+1}$, we have that 
	\begin{equation}\label{equ5}
	V^{\pi^{*}}(r,\widehat{P}^{k})-V^{\pi}(r,\widehat{P}^{k})\leq 2C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).
	\end{equation}
	Then we have
	\begin{align*}
	V^{\pi^{*}}(r,P)-V^{\pi}(r,P)&\leq |V^{\pi^{*}}(r,P)-V^{\pi^{*}}(r,\widehat{P}^{k})|+V^{\pi^{*}}(r,\widehat{P}^{k})-V^{\pi}(r,\widehat{P}^{k})+|V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,P)|\\ &\leq 4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).
	\end{align*}
	The last inequality is because of Lemma~\ref{lem16} and~\eqref{equ5} .
\end{proof}

\begin{lemma}\label{lem19}
	Conditioned on Lemma~\ref{lem16}, the total regret is at most $\widetilde{O}(\sqrt{H^{4}S^{2}AT})$.
\end{lemma}

\begin{proof}
	The regret for the first stage (stage 1) is at most $2HT^{(1)}=O(HK^{\frac{1}{2}})$. \\
	For stage $k\geq2$, the policies we use (any $\pi\in\phi^{k}$) are at most $4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k-1)}})$ sub-optimal, so the regret for the k-th stage is at most
	$8CT^{(k)}(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k-1)}}).$ \\
	Adding up the regret for each stage , we have that the total regret is bounded by
	\begin{align*}
	Regret(T)&\leq 2HK^{\frac{1}{2}}+\sum_{k=2}^{K_{0}}8CT^{(k)}(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k-1)}}) \\ &= O(HK^{\frac{1}{2}})+ O(\sqrt{H^{5}S^{2}A\iota K}\cdot \log\log(K))+O(S^{3}A^{2}H^{5}\iota K^{\frac{1}{4}})\\ &= O(\sqrt{H^{5}S^{2}A\iota K}\cdot \log\log(K))+O(S^{3}A^{2}H^{5}\iota K^{\frac{1}{4}}) \\ &= \widetilde{O}(\sqrt{H^{4}S^{2}AT}).
	\end{align*}
\end{proof}

Then Theorem~\ref{the1} holds because of Lemma~\ref{lem15} and Lemma~\ref{lem19}.

\begin{corollary}[Restate Corollary~\ref{co1}]
	Under the same assumption as Theorem~\ref{the1}, for any $\epsilon >0$, Algorithm~\ref{algo3} can output a stochastic policy $\widehat{\pi}$ such that with high probability, $$V_{1}^{*}(s_{1})-V_{1}^{\widehat{\pi}}(s_{1})\leq \epsilon$$ after $K=\widetilde{O}(\frac{H^{5}S^{2}A}{\epsilon^{2}})$ episodes.
\end{corollary}

\begin{proof}
	By Theorem~\ref{the1}, we have that the regret is bounded by $\widetilde{O}(\sqrt{H^{4}S^{2}AT})$ with high probability, which means we have
	$$\sum_{k=1}^{K}V_{1}^{*}(s_{1})-V_{1}^{\pi_{k}}(s_{1})\leq \widetilde{O}(\sqrt{H^{4}S^{2}AT}),$$ where $\pi_{k}$ is the policy used in episode $k$. Now define a stochastic policy $\widehat{\pi}$ as 
	$$\widehat{\pi}=\frac{1}{K}\sum_{k=1}^{K}\pi_{k}.$$
	Then we have
	$$\mathbb{E}[V_{1}^{*}(s_{1})-V_{1}^{\widehat{\pi}}(s_{1})]=\frac{1}{K}\sum_{k=1}^{K}V_{1}^{*}(s_{1})-V_{1}^{\pi_{k}}(s_{1})\leq \widetilde{O}(\sqrt{\frac{H^{5}S^{2}A}{K}}).$$
	By Markov inequality, we have with high probability that 
	$$V_{1}^{*}(s_{1})-V_{1}^{\widehat{\pi}}(s_{1})\leq \widetilde{O}(\sqrt{\frac{H^{5}S^{2}A}{K}}).$$
	Taking $K=\widetilde{O}(\frac{H^{5}S^{2}A}{\epsilon^{2}})$ bounds the above by $\epsilon$.
\end{proof}

\section{Proof of lower bound (Theorem~\ref{the2})}\label{appd}
\begin{theorem}[Restate Theorem~\ref{the2}]
	When $S\leq A^{\frac{H}{2}}$, for any algorithm with sub-linear regret bound, the global switching cost is at least $\Omega(HSA)$.
\end{theorem}
For the $\Omega(HSA)$ lower bound, we construct a MDP to show that it is at least as difficult as multi-armed bandit with $\Omega(HSA)$ arms. \citet{bai2019provably} proved an $\Omega(HSA)$ lower bound for local switching cost, which can only imply an $\Omega(A)$ lower bound for global switching cost in the worst case. In \cite{towards}, the authors proved an $\Omega(dH)$ lower bound for global switching cost under linear setting for all algorithms with PAC bound. The same lower bound is derived in \cite{gao2021provably} for all  algorithms with sub-linear regret. However, for the MDPs constructed by both papers, the number of actions available at each state is not the same, which means we can not get an $\Omega(HSA)$ lower bound by directly plugging in $d=SH$. Finally, an $\Omega(HSA)$ lower bound on global switching cost is the optimal result for any no-regret algorithms. This is because we can run our low adaptive reward-free exploration (Algorithm~\ref{algo4}) for $K^{\frac{2}{3}}$ episodes and run the policy $\widehat{\pi}^{r}$ where $r$ is the real reward function for the remaining episodes. It can be shown that the regret is of order $O(T^{\frac{2}{3}})$ and global switching cost is bounded by $2HSA$.

\begin{proof}
In this part of proof, we will add a mild assumption to parameters $H,S,A$. We assume that $S\leq A^{\frac{H}{2}}$. First we will show that under this assumption, a MDP with $S$ states, $A$ actions and horizon $H$ can be at least as difficult as a multi-armed bandit with $\Omega(HSA)$ arms.

We will consider a MDP will $S$ states, $A$ actions and horizon $H$. The initial state is fixed as $s_{0}$. The MDP can be divided into three parts.
\paragraph{Absorbing state}
There exists an absorbing state $s^{\dagger}$, such that for any action $a$ and $h\in[H]$, $P_{h}(s^{\dagger}|s^{\dagger},a)=1$ while $P_{h}(s|s^{\dagger},a)=0$ for any $s\neq s^{\dagger}$. The reward is defined as $r_{h}(s^{\dagger},a)=0$ for any $a,h\in[H]$.

\paragraph{The first several layers}
Let $H_{0}$ be the minimal positive integer such that $S\leq A^{H_{0}}$. By the assumption we have $H_{0}\leq \frac{H}{2}$. Then we can use an $A$-armed tree structure to ensure that for any state $s$, there exists a unique path starting from $s_{0}$ to arrive at $(H_{0},s)$. There are $S$ such paths altogether, and there may be some pairs $(H_{0}-1,s,a)$ that won't be used. For such pairs, we just  let $P_{H_{0}-1}(s^{\dagger}|s,a)=1$. The reward $r_{h}$ is always $0$ when $h\leq H_{0}-1$.

\paragraph{The remaining layers}
For each state $s$ and $h\geq H_{0}$, there exists a single action $a_{s,h}$ such that $P_{h}(s|s,a_{s,h})=1$ while $P_{h}(s^{\prime}|s,a_{s,h})=0$ for $s^{\prime}\neq s$. For any $a\neq a_{s,h}$, we have that $P_{h}(s^{\dagger}|s,a)=1$. The reward function  $r_{h}(s,a_{s,h})=0$ when the action is the $a_{s,h}$ that keeps the agent at $s$, and the reward for other actions $r_{h}(s,a)$ is unknown when $h\geq H_{0}$, $a\neq a_{s,h}$.

We can see that under this MDP, there are two cases. The first one is the agent arrives at $(H_{0},s^{\dagger})$ with no reward. The second one is the agent arrives at some $(H_{0},s)$ and finally arrives at $s^{\dagger}$ from the tuple $(h,s,a)$ ($h\geq H_{0}$ and $a\neq a_{s,h}$) with total reward $r_{h}(s,a)$. Also, for any deterministic policy, the trajectory is fixed, like pulling an 'arm' in bandit setting. Note that the total number of such 'arm's is at least $(S-1)(A-1)\frac{H}{2}\geq \Omega(HSA)$. Even if the transition structure is known to the agent, this MDP is still as difficult as a multi-armed bandit problem with $\Omega(HSA)$ arms. Then because any algorithm with sub-linear regret for multi-armed bandits needs to at least pull each arm once, we directly prove the theorem.
\end{proof}

\section{Proof of lemmas in low adaptive reward-free exploration}\label{appe}
\begin{lemma}\label{lem20}
	The total global switching cost of Algorithm~\ref{algo4} is bounded by $2HSA$.
\end{lemma}

\begin{remark}
The switching cost $O(HSA)$ is optimal for reward-free setting. With the same construction as the MDP in Appendix~\ref{appd}, we can show that it takes $\Omega(HSA)$ switching cost to find out the mapping between the policy and which arm it is pulling.
\end{remark}

Recall that $\iota=\log(2HAK/\delta)$.
\begin{lemma}\label{lem21}
	For any $\epsilon >0$, there exists $C>0$, when $N_{0}>C\cdot\frac{S^{3}AH^{5}\iota}{\epsilon}$, we have with probability $1-\frac{\delta}{2}$, for any $\pi\in\phi^{1}$ and any reward function $r$, $|V^{\pi}(r,P)-V^{\pi}(r,\widetilde{P})|\leq\frac{\epsilon}{4}$.
\end{lemma}

\begin{proof}
	This is a direct inference of lemma~\ref{lem10}.
\end{proof}

\begin{lemma}\label{lem22}
	For any $\epsilon >0$, there exists $C>0$, when $N>C\cdot \frac{H^{5}S^{2}A\iota}{\epsilon^{2}}$, with probability $1-\delta$, for any $\pi\in\phi^{1}$ and reward function $r$, $|V^{\pi}(r,\widehat{P})-V^{\pi}(r,\widetilde{P})|\leq\frac{\epsilon}{4}$.
\end{lemma}

\begin{proof}
	This is a direct inference of Lemma~\ref{lem14}.
\end{proof}

\begin{lemma}\label{lem23}
	For any $\epsilon >0$, there exists $C>0$, when the total episodes $K=N_{0}+N>C\cdot (\frac{H^{5}S^{2}A\iota}{\epsilon^{2}}+\frac{S^{3}AH^{5}\iota}{\epsilon})$, with probability $1-\delta$, for any $\pi\in\phi^{1}$ and reward function $r$, $|V^{\pi}(r,\widehat{P})-V^{\pi}(r,P)|\leq\frac{\epsilon}{2}$.
\end{lemma}

\begin{proof}
This lemma is a direct inference of $|V^{\pi}(r,\widehat{P})-V^{\pi}(r,P)|\leq|V^{\pi}(r,\widehat{P})-V^{\pi}(r,\widetilde{P})|+|V^{\pi}(r,\widetilde{P})-V^{\pi}(r,P)|$, Lemma~\ref{lem21} and Lemma~\ref{lem22}.
\end{proof}

\begin{lemma}\label{lem24}
	Conditioned on the case in Lemma~\ref{lem23}, we have that $0\leq V^{\pi^{*}}(r,P)-V^{\widehat{\pi}^{r}}(r,P)\leq \epsilon$ holds for any reward function $r$.
\end{lemma}

\begin{proof}
	$V^{\pi^{*}}(r,P)-V^{\widehat{\pi}^{r}}(r,P)\geq 0$ is obvious. Also,
	\begin{align*}
	V^{\pi^{*}}(r,P)-V^{\widehat{\pi}^{r}}(r,P)&\leq |V^{\pi^{*}}(r,P)-V^{\pi^{*}}(r,\widehat{P})|+V^{\pi^{*}}(r,\widehat{P})-V^{\widehat{\pi}^{r}}(r,\widehat{P})+|V^{\widehat{\pi}^{r}}(r,\widehat{P})-V^{\widehat{\pi}^{r}}(r,P)|\\ &\leq \epsilon.
	\end{align*}
	The second inequality is because of Lemma~\ref{lem23} and $\widehat{\pi}^{r}=argmax_{\pi\in\phi^{1}}V^{\pi}(r,\widehat{P})$.
\end{proof}

Then Theorem~\ref{the3} holds because of Lemma~\ref{lem20} and Lemma~\ref{lem24}.


\section{Improved algorithm with near optimal adaptivity}\label{appi}
\begin{algorithm}
	\caption{Adaptive Policy Elimination by Value Estimation+ (APEVE+)}\label{algo6}
	\begin{algorithmic}[1]
		\STATE \textbf{Require}: Number of episodes for exploration $K$, $r$ is the known deterministic reward. Universal constant $C$. Failure probability $\delta$.
		\STATE \textbf{Initialize}: $T^{(k)}=K^{1-\frac{1}{2^{k}}}$, $k\leq K_{0}=O(\log\log K)$, $\phi^{1}:=\{ \text{the set of all the deterministic policies}\}$, $\iota=\log(2HAK/\delta)$. %($A^{SH}$ policies altogether). 
		\FOR{$k=1,2,\cdots,K_{0}$}  
		\STATE \maroon{$\diamond$ Number of episodes in $k$-th stage:}
		\IF{$T^{(1)}+T^{(2)}+\sum_{i=1}^{k}T^{(i)}\geq K$} 
		\STATE $T^{(k)}=K-T^{(1)}-T^{(2)}-\sum_{i=1}^{k-1}T^{(i)}$. (o.w. $T^{(k)}=K^{1-\frac{1}{2^{k}}}$)
		\ENDIF
		\ENDFOR
		\STATE \maroon{Adaptive policy elimination for the first two stages:}
		\FOR{$k=1,2$}
		\STATE \maroon{Update the infrequent set $\mathcal{F}^{k}$ and construct empirical estimate of the absorbing MDP:}
		\STATE $\mathcal{F}^{k}$,$P^{int,k}$ = Exploration$(\phi^{k},T^{(k)}).$
		\STATE $\widehat{P}^{k}$ = Evaluation$(\mathcal{F}^{k},P^{int,k},T^{(k)},\phi^{k}).$
		\STATE $U^k=\emptyset$ 
		\FOR{$\pi\in\phi^{k}$}
		\IF{$V^{\pi}(r,\widehat{P}^{k})\leq sup_{\widehat{\pi}\in\phi^{k}}V^{\widehat{\pi}}(r,\widehat{P}^{k})-2C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}})$}
		\STATE Update $U^{k}\leftarrow U^k\cup \{\pi\}$.
		\ENDIF
		\ENDFOR
		\STATE $\phi^{k+1}\leftarrow\phi^{k}\backslash U^k$.
		\ENDFOR
		\STATE \maroon{Adaptive policy elimination for the remaining stages:}
		\FOR{$k=3,4,\cdots,K_{0}$}
		\STATE \maroon{Keep the infrequent set $\mathcal{F}^{2}$ and construct empirical estimate of the absorbing MDP with new data set:}
		\STATE $\widehat{P}^{k}$ = Evaluation$(\mathcal{F}^{2},P^{int,2},T^{(k)},\phi^{k}).$
		\STATE $U^k=\emptyset$ 
		\FOR{$\pi\in\phi^{k}$}
		\IF{$V^{\pi}(r,\widehat{P}^{k})\leq sup_{\widehat{\pi}\in\phi^{k}}V^{\widehat{\pi}}(r,\widehat{P}^{k})-2C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}})$}
		\STATE Update $U^{k}\leftarrow U^k\cup \{\pi\}$.
		\ENDIF
		\ENDFOR
		\STATE $\phi^{k+1}\leftarrow\phi^{k}\backslash U^k$.
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

We change APEVE (Algorithm~\ref{algo3}) slightly to get this APEVE+ (Algorithm~\ref{algo6}). The main difference is that only the first two stages contain the use of Exploration (Algorithm~\ref{algo1}), the remaining stages only run Evaluation (Algorithm~\ref{algo2}) and eliminate policy at the end of each stage. First, we consider the number of batches. Note that one application of Exploration can be finished in $H$ batches, because the exploration of each layer can be finished in one batch. Besides, one application of Evaluation can be finished in one batch. In Algorithm~\ref{algo6}, there are two applications of Exploration and $O(\log\log T)$ applications of Evaluation, so we have the following theorem.

\begin{theorem}\label{the77}
APEVE+ (Algorithm~\ref{algo6}) can be applied in $O(2H+\log\log T)=O(\log\log T)$ batches.
\end{theorem}

\begin{remark}
\citet{gao2019batched} proved that for any algorithm with $\widetilde{O}(\sqrt{T})$ regret bound under multi-armed bandit setting, the number of batches is at least $\Omega(\log\log T)$. In the construction of our lower bound in Appendix~\ref{appd}, we show that tabular RL can be at least as difficult as a multi-armed bandit problem, which means the $\Omega(\log\log T)$ lower bound on batches also applies to tabular RL setting. According to Theorem~\ref{the77}, we conclude that our Algorithm~\ref{algo6} matches the lower bound of batches.
\end{remark}

Now we will consider the regret bound of APEVE+. Same to Lemma~\ref{lem16}, we have the following key lemma.
\begin{lemma}
There exists a constant $C$, such that conditioned on the cases in Lemma~\ref{lem10} ($k=1,2$) and Lemma~\ref{lem14} (all $k$), for any $k=1,2$ and $\pi\in\phi^{k}$, we have 
	$$|V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,P)|\leq C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}).$$
	Also, for any $k\geq 3$ and $\pi\in\phi^{k}$, we have $$|V^{\pi}(r,\widehat{P}^{k})-V^{\pi}(r,P)|\leq C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}}).$$
	In addition, the probability of this case is at least $1-\delta$.
\end{lemma}

Then using the same proof as Lemma~\ref{lem17} and Lemma~\ref{lem18}, we have an upper bound on the sub-optimality of policies used in each stage.

\begin{lemma}
	With probability $1-\delta$, for the policies that have not been eliminated at stage $k$, i.e. $\pi\in\phi^{k+1}$, we have that
	$$V^{\pi^{*}}(r,P)-V^{\pi}(r,P)\leq 4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(k)}}),\ k=1,2.$$
	$$V^{\pi^{*}}(r,P)-V^{\pi}(r,P)\leq 4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}}),\ k\geq 3.$$
\end{lemma}

Now we are ready to bound the total regret of Algorithm~\ref{algo6}.
\begin{theorem}
With probability $1-\delta$, the total regret of APEVE+ (Algorithm~\ref{algo6}) is at most $\widetilde{O}(\sqrt{H^{4}S^{2}AT})$.
\end{theorem}

\begin{proof}
	The regret for the first stage (stage 1) is at most $2HT^{(1)}=O(HK^{\frac{1}{2}})$. \\
	The regret for the second stage (stage 2) is at most $2T^{(2)}\times4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(1)}}}+\frac{S^{3}A^{2}H^{5}}{T^{(1)}})$. \\
	For stage $k\geq3$, the policies we use (any $\pi\in\phi^{k}$) are at most $4C(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}})$ sub-optimal, so the regret for the k-th stage is at most
	$8CT^{(k)}(\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}}).$ \\
	Adding up the regret for each stage , we have that the total regret is bounded by
	\begin{align*}
	Regret(T)&\leq 2HK^{\frac{1}{2}}+\sum_{k=2}^{K_{0}}8CT^{(k)}\sqrt{\frac{H^{5}S^{2}A\iota}{T^{(k-1)}}}+8CT^{(2)}\frac{S^{3}A^{2}H^{5}\iota}{T^{(1)}}+\sum_{k=3}^{K_{0}}8CT^{(k)}\frac{S^{3}A^{2}H^{5}\iota}{T^{(2)}} \\ &= O(HK^{\frac{1}{2}})+ O(\sqrt{H^{5}S^{2}A\iota K}\cdot \log\log(K))+O(S^{3}A^{2}H^{5}\iota K^{\frac{1}{4}})\\ &= O(\sqrt{H^{5}S^{2}A\iota K}\cdot \log\log(K))+O(S^{3}A^{2}H^{5}\iota K^{\frac{1}{4}}) \\ &= \widetilde{O}(\sqrt{H^{4}S^{2}AT}).
	\end{align*}
\end{proof}
\end{onecolumn}













==> sections/simulation.tex <==
% !TEX root = ../example_paper.tex

Under non-Markov setting, the agent is allowed to use a mixture of deterministic policies. Our algorithms can be used under this setting with a natural modification. Recall that in Exploration (Algorithm~\ref{algo1}), for each layer $h$, we apply each $\pi_{h,s,a}$ ($(s,a)\in \mathcal{S}\times\mathcal{A}$) for the same number of episodes $\frac{T}{HSA}$. If we apply a mixture of all these $\pi_{h,s,a}$, which defined as $\pi_{h}$ such that $\pi_{h}=\pi_{h,s,a}$ with probability $\frac{1}{SA}$, then we can apply $\pi_{h}$ for $\frac{T}{H}$ episodes instead. The algorithm will have the same exploration effect with global switching cost only $H$. Using the same idea, in Evaluation (Algorithm~\ref{algo2}), we can apply $\pi_{random}$ that chooses each $\pi_{h,s,a}$ with probability $\frac{1}{HSA}$, $\forall\,(h,s,a)\in[H]\times \mathcal{S}\times\mathcal{A}$. Then the global switching cost for Algorithm~\ref{algo2} will be only $1$. Under a new schedule of Exploration and Evaluation, we have the following result.
\begin{theorem}\label{the6}
Under non-Markov setting, Algorithm~\ref{algo5} can achieve $\widetilde{O}(\sqrt{H^{4}S^{2}AT})$ regret while global switching cost is bounded by $2H+O(\log\log T)$.
\begin{remark}
We can see that under non-Markov setting, we can save a factor of $HSA$ for global switching cost.
\end{remark}
\end{theorem}
